Multi-Agent Cooperation and the Emergence of (Natural) Language

The current mainstream approach to train natural language systems is to expose them to large amounts of text. This passive learning is problematic if we are interested in developing interactive machines, such as conversational agents. We propose a framework for language learning that relies on multi-agent communication. We study this learning in the context of referential games. In these games, a sender and a receiver see a pair of images. The sender is told one of them is the target and is allowed to send a message from a fixed, arbitrary vocabulary to the receiver. The receiver must rely on this message to identify the target. Thus, the agents develop their own language interactively out of the need to communicate. We show that two networks with simple configurations are able to learn to coordinate in the referential game. We further explore how to make changes to the game environment to cause the "word meanings" induced in the game to better reflect intuitive semantic properties of the images. In addition, we present a simple strategy for grounding the agents' code into natural language. Both of these are necessary steps towards developing machines that are able to communicate with humans productively.

==> OLD/experiments.tex <==
\section{Learning to Communicate}
\label{sec:exp1}

Our first question is whether agents converge to successful
communication at all. To test this, we run them through a training
phase of 50k rounds of play and report test performance after each
round. Figure \ref{fig:exp1_comm} plots the communicative success
(i.e., proportion of test plays in which the agents successfully
coordinated) as a function of training rounds. We see that our agents
do indeed converge to communication, approaching their asymptotes
after about 1.5K rounds. These results are robust to changing various parameters of the game (sender architecture, image representation, vocabulary size).%with an average success rate of 94$\%$ across
%models.\COMMENT{is this with probs or fc representations?}


\begin{figure}[tb]
\centering
\includegraphics[scale=0.4]{figures/fc}
\caption{Communication success as a function of training iterations for the configurations using fc visual representations.}
\label{fig:exp1_comm}
\end{figure}



% \begin{table}
% \centering
% \begin{tabular}{c|c|c|c|c|c|c|c}
% visual representation&vocab size & used words& sender & commun. success &purity & rand. purity & purity-rand. purity\\\hline
% probs & 100 & 58 & shared & 1.00 & 0.46        & 0.27 & 0.19\\
% fc & 100 & 38 & shared & 1.00 & 0.41           & 0.23 & 0.18\\
% probs & 10 & 10 & shared & 1.00 & 0.35         & 0.18 & 0.18\\
% fc & 10 & 10 & shared & 1.00 & 0.32            & 0.17 & 0.14\\
% probs & 100 & 2 & fullyconnected & 0.99 & 0.21 & 0.15 & 0.06\\
% fc & 10 & 2 & fullyconnected & 0.99 & 0.21     & 0.15 & 0.05\\
% probs & 10 & 2 & fullyconnected & 0.99 & 0.20  & 0.15 & 0.04\\
% fc & 100 & 2 & fullyconnected & 0.99 & 0.19    & 0.15 & 0.04\\
% \end{tabular}
% \label{tab:exp1_table}
% \caption{Table with results, no noise}
% \end{table}

\begin{table}
\centering
\begin{tabular}{c|c|c|c|c|c|c|c}
id & sender   &vis   &voc &used     &comm    &      purity ($\%$)   &obs-chance\\
 	&	& rep & size& symbols & success($\%$) &  & purity ($\%$) \\\hline
1&informed&probs     &100       &58          &100                &46           &0.27 \\
2&informed&fc        &100       &38          &100                &41           &0.23 \\
3&informed&probs     &10        &10          &100                &35           &0.18 \\
4&informed&fc        &10        &10          &100                &32           &0.17 \\
5&agnostic&probs     &100       &2           &99                 &21           &0.15 \\
6&agnostic&fc        &10        &2           &99                 &21           &0.15 \\
7&agnostic&probs     &10        &2           &99                 &20           &0.15 \\
8&agnostic&fc        &100       &2           &99                 &19           &0.15 \\
\end{tabular}
\label{tab:exp1_table}
\caption{Playing the referential game. \emph{Used symbols} column reports number of distinct vocabulary symbols that were produced at least once in the test phase. See text for explanation of \emph{comm success} and \emph{purity}. All purity values are highly significant ($p<0.001$) compared to simulated chance symbol assignment when matching observed symbol usage. %\textbf{Is this indeed the case? that is, is observed purity above the max chance value for all experiments reported in this table? if not, update accordingly. AL: YES, but I measured in your perl simulations how many times the chance purity was over the observed one.} 
The \emph{obs-chance purity} column reports the difference between observed purity and expected purity under chance.}
\end{table}

Table~\ref{tab:exp1_table} shows communication success for various configurations after 5k training rounds. Both sender architectures learn
to coordinate with the receiver. However, they have very different
qualitative behavior.  The informed sender, being encouraged to detect
pairwise relations between images, tends to make use of more symbols
from the available vocabulary, while the sender without this feature
coordinates using a very compact vocabulary. This might suggest that
the informed sender is using more varied and word-like symbols (recall
that the images depict about 463 objects, so we would expect a
natural-language-endowed sender to use a wider array of symbols to
discriminate among them). However, it could also be the case that the
informed sender vocabulary simply contains higher
redundancy/synonymy. Figure~\ref{fig:exp1_synonymy} plots the singular
values and spectral clustering of the informed sender symbol usage
(with fc input representations and 100 as  symbol vocabulary
size). We observe that, while there is some redundancy, the vocabulary
would not be able to get reduced to two symbols with the current
communication protocol.
\COMMENT{I did not follow the line of reasoning here: isn't the fact that the vocabulary could be reduced to two singular values a sign that it's indeed very redundant?} AL: Why do you  say that the vocabulary can be reduced to two symbols only? There is some information carried by the other dimensions as well.

\begin{figure}[tb]
\centering
\includegraphics[scale=0.35]{figures/singular}
\caption{Singular values and spectral clustering of symbols}
\label{fig:exp1_synonymy}
\end{figure}

\COMMENT{I am commenting out the
  former description and replacing it with one of what I did. Alex: if
  the description that follows is wrong, please reinstate yours.}

We now turn to investigating the semantic properties of the emergent
communication protocol. Recall that the vocabulary that agents use is
arbitrary and has no initial meaning. Thus, one way to look for the
emergence of high (vs.~low) level semantics is to look for the
relationship between symbols and the sets of images they refer to. To
look for these higher-level properties, we exploit the fact that the
objects in our images were categorized into \textbf{10} \textbf{AL: Why 10? We have 20...} broader
categories (such as \emph{weapon} and \emph{mammal}) by
\cite{McRae:etal:2005}. If the agents converged to intuitive meanings
for the symbols, we would expect that objects belonging to the same
category would activate the same symbols, e.g., that, say, when the
target images depict bayonets and guns, the sender would use the same
symbol to signal them. To quantify this, we associate each object to
the symbol that is most often activated when the target images contain
the object. We then assess the quality of the resulting symbol-based
clusters by measuring their \emph{purity} with respect to the McRae
categories. Purity \citep{Zhao:Karypis:2001} is a standard measure of
cluster quality, reaching 100\% for perfect clustering with respect to
the gold standard, and approaching 0 as cluster quality deteriorates.

Although purity is far from perfect, it is significantly above chance
in all cases, and we confirm that the informed-sender is producing
symbols that are more semantically natural than those of the agnostic
one. Perhaps surprisingly, purity is not at chance level even when
only two symbols are used. Qualitatively, in this case the agents seem
to converge to a (noisy) living-vs-non-living distinction, which,
intriguingly, has been recognized as the most basic one in the human
semantic system \citep{Caramazza:Shelton:1998}.

% We then compare this to the expected purity that we would get if class labels were randomly assigned to images. We see that the purity is higher than random, but that the clusters are not completely pure. 

% It is hard to interpret this measure as an absolute one, but we will show in our next experiment that interventions which we expect to raise the utilization of higher order features do, in fact, raise this measure as well.


% ALEX FROM HERE
% We now turn to investigating the natural language properties of the
% emergent communication protocol. Recall that the vocabulary that
% agents use is arbitrary and has no initial meaning. Thus, one way to
% look for the emergence of high (vs.~low) level semantics is to look
% for the relationship between symbols and the images they refer
% to.

% %[Discuss number of words used and whether that is necessarily high vs. low level]
% To look for these higher-level properties, we exploit the fact that
% each image that we work with already has an ImageNet class and there
% are many images in our set from each class. The basic idea is to ask
% whether we can use higher-level attributes of the image (e.g., whether
% the image is depicting a cat) to predict which vocabulary word the
% agents use to refer to it. If the agents are using low-level features
% (e.g., brightness in certain areas of the image), then we should be
% unable to do so.

% For every image, we look at the most commonly used word when that image is the target. We then treat the ImageNet class (eg. chair, fox, butterfly) as a clustering of images and compute the purity of the cluster by

% %[purity equation here]

% We then compare this to the expected purity that we would get if class labels were randomly assigned to images. We see that the purity is higher than random, but that the clusters are not completely pure. 

% It is hard to interpret this measure as an absolute one, but we will show in our next experiment that interventions which we expect to raise the utilization of higher order features do, in fact, raise this measure as well.
% ALEX TO HERE

\COMMENT{Assuming my description above is correct, I think the
  following is a different experiment, and this should be clarified}

We can visualize the clustering patterns as follows. For every
ImageNet class, we look at the symbol most commonly used by the sender
when an image of that class is the target. In addition, for each
class, we generate an embedding by averaging the embeddings of each
image in the class. We think this captures higher-level class
semantics for two reasons: first, the top layers of convolutional
neural networks are often thought to be expressing quite high-level
features of images \citep{Zeiler:Fergus:2014}. Second, if lower-level
features (e.g., brightness) are randomly assigned within class then
this averaging removes lower-level signals and leaves only higher
level ones.

\COMMENT{I don't understand the line of reasoning above. The aim of the current analysis is to show that the agents are converging to a meaningful code. In this perspective, what is the point of trying to use an external mechanism that is not part of agent's communication, namely averaging across images of objects? I think the latter should simply be justified as a way to improve the visualization, and not in virtue of any denoising function they might have. Perhaps, it would be even better to plot single images randomly selected?}

We then take these class embeddings and inspect if they form natural clusters and whether these clusters align with word usage. To see this, we perform a t-SNE mapping~\cite{Laurens:Hinton:2008} of the class embedding matrix, color-coded  by their majority symbol used. Figure \ref{fig:exp1_tsne} shows the result.

%\COMMENT{These plots should feature labels for a subset of the points, to let the reader understand what's going on.}

\begin{figure}[tb]
\centering
\includegraphics[scale=0.39]{figures/informed_fc_10_v1n0}
\includegraphics[scale=0.39]{figures/informed_fc_10_v1n1}
\caption{t-SNE plots of configurations without noise (\textbf{left}, 4th row of Table~\ref{tab:exp1_table}) and with noise (\textbf{right}, 2nd row of Table~\ref{tab:exp2_multiinstance}).}
\label{fig:exp1_tsne}
\end{figure}




\section{Learning Higher-Level Semantics}
\label{sec:exp2}

We established that our agents can solve the coordination problem, and
we have at least tentative evidence that they do so by developing
symbol meanings that align with our semantic intuition. We turn now to
a simple way to tweak the game setup in order to encourage the agents
to further pursue high-level semantics.

Specifically, we remove some aspects of ``common knowledge'' from the game. Common knowledge, in game theoretic parlance, are facts that everyone knows, everyone knows that everyone knows, everyone knows that everyone knows that everyone knows and so on (\cite{brandenburger2014hierarchies}). Coordination can only occur if the basis of the coordination is common knowledge (\cite{rubinstein1989electronic}), therefore if we remove some common knowledge, we will preclude our agents from coordinating on these facts. In our case, we will remove from common knowledge facts pertaining to the details of the input images, thus forcing the agents to coordinate on more abstract properties.

At the same time, we aim to simulate real reference scenarios more
closely.  In the simulations of Section~\ref{sec:exp1}, both agents
had access to the exact same visual representation of each
image. However, this is a highly suspect assumption. If we imagine two
humans playing this game, there are many reasons we should expect them
to have different interpretations of each object. At a simple physical
level, they will not have the same viewpoint of the object (and this
alone will alter low-level properties such as illumination). At a
higher cognitive level, each of us has unique interaction histories
with the world as well as differences in our biology (e.g.,
color-blindness) and so we perceive and interpret things in different
ways \cite{}.

We thus remove low-level common knowledge by letting the agents playing the game at the ImageNet class level, by showing them different images
belonging to the same class (e.g., if the target is \emph{dog}, the
sender is shown a picture of a Chihuahua and the receiver that of a
Boston Terrier).

% \begin{table}[tb]
% \centering
% \begin{tabular}{c|c|c|c|c|c|c|c}
% visual representation&vobab size & used words& sender & commun. success &purity & rand. purity & purity-rand. purity\\\hline
% fc & 100 & shared & 43 & 1.00 & 0.45 & 0.24 & 0.21\\
% %probs & 10 & shared & 10 & 0.99 & 0.37 & 0.18 & 0.20\\
% fc & 10 & shared & 10 & 1.00 & 0.37 & 0.18 & 0.19\\
% %probs & 100 & shared & 62 & 0.99 & 0.46 & 0.28 & 0.18\\
% fc & 10 & fullyconnected & 3 & 0.98 & 0.28 & 0.16 & 0.12\\
% %probs & 10 & fullyconnected & 2 & 0.94 & 0.22 & 0.15 & 0.07\\
% fc & 100 & fullyconnected & 2 & 0.92 & 0.23 & 0.15 & 0.07\\
% %probs & 100 & fullyconnected & 2 & 0.93 & 0.22 & 0.15 & 0.06\\
% \end{tabular}
% \caption{Table with results, multiple instance noise}
% \label{tab:exp2_multiinstance}
% \end{table}

\begin{table}[tb]
\centering
\begin{tabular}{c|c|c|c|c|c|c|c}
id &sender   &vis   &voc &used     &comm    &      purity ($\%$)   &obs-chance\\
 &		& rep & size& symbols & success($\%$) &  & purity ($\%$) \\\hline
1&informed&fc      &100     &43          &1.00               &0.45         &0.21\\
2&informed&fc      &10      &10          &1.00               &0.37         &0.19\\
3&agnostic&fc      &100     &2           &0.92               &0.23         &0.07\\
4&agnostic&fc      &10      &3           &0.98               &0.28         &0.12\\
\end{tabular}
\caption{Playing the referential game with image-level targets. Columns as in Table \ref{tab:exp1_table}. All purity values significant at $p<0.001$.}
\label{tab:exp2_multiinstance}
\end{table}

Table~\ref{tab:exp2_multiinstance} presents the results in various
configurations. We see that the agents are still able to
coordinate. Moreover, we observe a small increase in symbol usage
purity, as expected since agents can now only coordinate on general
properties of concept classes, rather than on the specific properties
of each image. This effect emerges even more clearly in Figure
~\ref{fig:exp1_tsne}, reporting a t-SNE based visualization of
average class embeddings as they emerge in the modified game.

\COMMENT{I have tentatively commented out the discussion of the cross-layer strategy, since it doesn't seem to improve purity, and the table was already commented out. Feel free to reinstate.}

% While effective, the aforementioned  training curriculum requires access to image object annotations and is a bit artificial. A less knowledge-intensive technique for removing low-level common knowledge is to present agents with different representations of the same image. 

% This can be achieved either by using, for the visual representation, a different network architecture or the same architecture trained differently (different seed or training data). 

% Here,  we adopt a simpler way and present agents with representations of the same image coming from the same network but from different layers, e.g., the sender's input representation of an image is the last layer while the receiver's is the second to last layer.  

% We note that this does not exactly remove common knowledge of low level features, since by definition the last layer is a (non-linear) transformation of previous ones. However, it does make coordination on one particular dimension, or simple function of several dimensions, of the embedding much more difficult. 

% Again, we find that this does not impede accuracy very much but does lead to an increase in the purity of our clusters - that is, words used to refer to entities become more predictable by higher level features of the image, eg. its class.

\iffalse
\begin{table}
\centering
\begin{tabular}{c|c|c|c|c|c|c|c}
visual representation&vobab size & used words& sender & commun. success &purity & rand. purity & purity-rand. purity\\\hline
fc & 100 & shared & 54 & 0.98 & 0.48 & 0.26 & 0.22\\
%probs & 100 & shared & 59 & 0.98 & 0.47 & 0.27 & 0.20\\
%probs & 10 & shared & 10 & 0.96 & 0.35 & 0.18 & 0.18\\
fc & 10 & shared & 10 & 0.97 & 0.29 & 0.18 & 0.11\\
%probs & 10 & fullyconnected & 2 & 0.88 & 0.25 & 0.15 & 0.09\\
fc & 10 & fullyconnected & 2 & 0.89 & 0.24 & 0.15 & 0.09\\
%probs & 100 & fullyconnected & 2 & 0.87 & 0.22 & 0.15 & 0.06\\
fc & 100 & fullyconnected & 2 & 0.90 & 0.21 & 0.15 & 0.05\\
\end{tabular}
\caption{Table with results, crosslayer noise}
\label{tab:exp2_crosslayer}
\end{table}
\fi


\section{Grounding Agents' Communication in Human Language}
The results in Section~\ref{sec:exp1} show that communication robustly
arises in our game across various parameters.  The clustering results
there and in Section~\ref{sec:exp2} suggest moreover that agents are
developing symbol meanings that are not, altogether, too different
from conventional word meanings: Symbols come to
denote broad conceptual properties, such as those that might
distinguish, say, buildings from vegetables, rather than, say,
low-level perceptual properties of images. Still, we would like to
actually make it so that the agents converge on words that
are fully understandable by humans, as our ultimate goal is to develop
machines that can hold conversations with us. %
%  However to ensure the emergence of
% human-understandable language, it is essential to ensure that agents
% will not ``drift'' into their own protocol. Agents which begin as
% tabulae rasae may converge to any ``word'' being used as a reference
% for any object.

% In section~\ref{sec:exp2} we partially increased the semantic coherence  of the communication protocol, however semantic coherence is not enough for our goals. In our current setup if the agent sender was to be replaced by a human, she would likely not be able to decipher the meaning of the symbols without a training phase, if at all. If we want to eventually train agents which can interact in novel environments and with humans we need to find ways to ground communication in not only high level semantic properties of the images, but also natural language.
We take inspiration from the recent success story of AlphaGo
\cite{Silver:etal:2016}, an AI that learned to play Go at the master
level by combining interactive learning in games of self-play with
passive supervised learning from a large set of human
games. Similarly, we combine the usual referential game, in which
agents interactively develop their communication protocol, with a
supervised image labeling task, where the sender must learn to assign
objects the same names that humans use. In this way, the sender will
naturally be encouraged to such names to discriminate the
target image when playing the referential game, making their
communication more transparent to humans. %
% We propose that one way to move forward in grounding communication in natural language is combining dynamic interactive learning with static statistical learning of patterns from association.  In the context of the specific referential game, our agents will let to evolve a communication protocol, which we will ground in natural language via a supervised task. In this way, the symbols will have a direct correspondence to natural language through the human readable labels used in the classification task. 
Note that the supervised objective does not aim at improving agents'
playing performance. Instead, supervision provides them with basic
grounding in natural language (in the form of image-label
associations), while concurrent interactive game playing should teach
them how to effectively use this grounding to communicate.

Specifically, we designed an experiment in which the sender switches,
equiprobably, between game playing and a supervised image
classification task. We use the informed sender, fc image
representations and a vocabulary size of 100. Supervised training is
based on 100 labels that are a subset of the object names in our
data-set (see Section \ref{sec:experimental-setup} above). When
predicting object names, the sender only uses the game-embedding layer
(second layer from bottom of the network in the middle of Figure
\ref{fig:players}) and the softmax layer (top layer). These layers are
shared across the two setups. The units of the shared softmax layer
will correspond to sender symbols during game playing and to object
names for image labeling. Consequently, the symbols produced in the
game can be interpreted by the corresponding object names acquired in
the supervised phase.

\COMMENT{Mention accuracy in image labeling? \textbf{AL: Do I really have to do this?:-( I measure perplexity and not accuracy... MB: Perplexity is OK: just something to clarify that the agent is learning something also in the image labeling phase.}}

As expected, the supervised objective has no negative effect on
communication success: the agents are still able to reach full
coordination after \textbf{10k} training trials.\COMMENT{Does this
  mean it takes twice as many iteration than when you don't use
  supervision? Or do the 10K trials also include the supervised ones?}
Importantly, now symbol purity dramatically increases to 70\% (the
obs-chance purity difference also increases to 37\%; compare these
values to those in tables \ref{tab:exp1_table} and
\ref{tab:exp2_multiinstance} above). The sender is moreover using a
much higher proportion of symbols than in any previous experiment
(88\%). Even more importantly, many symbols have now become directly
interpretable, thanks to their direct correspondence to
labels. Considering the \textbf{632} image pairs where the target gold
standard label corresponds to one of the labels that were used in the
supervised phase, in 47\% of these cases the sender produced exactly
the symbol corresponding to the correct supervised label for the
target image (chance: 1\%). \COMMENT{Can you give me access to this
  subset of data, including the cases where another image was used? I
  think there might be something interesting there\ldots Are these the data you pasted below, commented out? They are a bit obscure, can you explain?}

%%RESULTS
  %%%informed	fc	100	88	0.998022	0.695464362850972       0.373091
%%47.1
%link with images

Interestingly, the beneficial interpretability effect obtained by
encouraging the sender to assign a conventional meaning to symbols
extends to images that do not contain the objects involved in the
supervised phase. To clearly illustrate this point, we ran a follow-up
experiment in which, during training, the sender was again exposed (with
equal probability) to the same supervised classification objective as
above, but now the agents %
% We now  turn to  a more challenging setup  aiming at testing  whether this method scales beyond concepts for which supervision is provided. For this experiment, the sender again with probability $p=0.5$ is exposed to  the same  supervised object classification  as before. 
played the referential game on a different dataset, derived from
ReferItGame~\citep{Kazemzadeh:etal:2014}. In its general format,
ReferItGame contains annotations of bounding boxes in real images with
referring expressions produced by humans when playing the
game. % This makes the more challenging as the number of depicted objects grows a lot, bounding boxes do not always include salient information etc.
For our purposes, we constructed \textbf{XX} pairs by randomly
sampling two bounding boxes, to act as target and distractor.  Again,
the agents converged to perfect communication after 15k trials, and
this time used all 100 available symbols in some trial.

For each symbol used by the trained sender, we then randomly extracted
3 image pairs in which the sender picked that symbol and the receiver
pointed at the right target. For two symbols, only 2 pairs matched
these criteria, leading to a set of 298 image pairs.  Recall that, in
the current setup, each symbol is associated with a word (the
corresponding gold supervised label), so we annotated each pair with
the word corresponding to the symbol. Out of the 298 pairs, only 25
(8\%) included one of the 100 words among the corresponding referring
expressions in ReferItGame. So, in the large majority of
cases, the sender had to produce a word that could probably only indirectly
refer to what is depicted in the target image. %
%6 12507 17311 bagpipe set(['chair'])
%7 17193 25296 pheasant set(['chair'])
%10 2520 43760 chain set(['chair'])
%21 27623 41370 crocodile set(['chair'])
%26 41441 17293 pine set(['fence'])
%47 2714 3410 grape set(['door'])
%62 40271 42312 melon set(['fence'])
%95 25227 28021 courgette set(['fence'])
%101 36865 31277 crow set(['car'])
%123 31626 5695 cart set(['chair'])
%135 26423 37803 box set(['car'])
%182 14044 21946 projector set(['door'])
%183 16234 9592 projector set(['bike'])
%185 8220 41414 alligator set(['door'])
%192 39554 34635 frog set(['sweater'])
%197 31954 23484 raft set(['fence'])
%228 30306 3220 rabbit set(['cat'])
%254 24593 30759 seagull set(['pillow'])
%265 38925 22486 wand set(['car'])
%267 33142 6106 dolphin set(['shack'])
%276 42296 25269 airplane set(['lime'])
%286 37893 29106 lamb set(['fence'])
%288 15391 19156 hoe set(['car'])
%289 38559 37741 hoe set(['rabbit'])
%296 6514 7256 freezer set(['car', 'train'])
%0.0838926174497 25 0.0%
We prepared a crowdsourcing survey using the CrowdFlower
platform.\footnote{\url{https://www.crowdflower.com/}} For each pair,
participants where shown the two pictures and the sender-emitted word (see
examples in Figure \ref{fig:dolphin_fence}). The participants were
asked to pick the picture that they thought was most related to the
word. We collected 10 ratings for each pair.

\begin{figure}[tb]
\centering
\includegraphics[scale=0.4]{figures/dolphin-fence.pdf}
\caption{Example pairs from the ReferItGame set, with word produced by
  sender. Target images framed in green.}
\label{fig:dolphin_fence}
\end{figure}

We found that in 68\% of the cases the subjects were able to guess the
right image. A logistic regression predicting subject choice from
ground-truth target image position, with subject and word random
factors added to intercept to control for these sources of
variability, confirmed the highly significant correlation between the
true and guessed positions ($z=16.75$, $p<0.0001$). 

Looking at the results qualitatively, we found that very often
sender-subject communication succeeded when the sender established a
sort of ``metonymic'' link between the words in its possession and the
contents of an image. This is illustrated by the typical examples in
Figure \ref{fig:dolphin_fence}, where the sender produced
\emph{dolphin} to refer to a picture showing a stretch of sea, and \emph{fence} for a patch of land. Similar semantic shifts are a core characteristic of natural
language \citep[e.g.,][]{Pustejovsky:1995}, and thus 
subjects were, in many cases, able to successfully play the
referential game with our sender (10/10 subjects guessed the dolphin
target, and 8/10 the fence one).

Although the language developed by the agents will initially be very
limited and not perfectly overlapping with that of humans, if both
agents and humans possess the sort of flexibility displayed in this
last experiment, we might hope that, once humans enter the loop, the
noisy but shared common ground will suffice to establish basic
communication, building on which humans could then further educate
machines.










==> figures/experiment1.tex <==
\section{Learning to Communicate}
\label{sec:exp1}

Our first question is whether agents converge to successful
communication at all. To test this, we run them through a training
phase of 50k rounds of play and report test performance after each
round. Figure \ref{fig:exp1_comm} plots the communicative success
(i.e., proportion of test plays in which the agents successfully
coordinated) as a function of training rounds. We see that our agents
do indeed converge to communication, approaching their asymptotes
after about 1.5K rounds. These results are robust to changing various parameters of the game (sender architecture, image representation, vocabulary size).%with an average success rate of 94$\%$ across
%models.\COMMENT{is this with probs or fc representations?}


\begin{figure}[tb]
\centering
\includegraphics[scale=0.4]{figures/fc}
\caption{Communication success as a function of training iterations for the configurations using fc visual representations.}
\label{fig:exp1_comm}
\end{figure}



% \begin{table}
% \centering
% \begin{tabular}{c|c|c|c|c|c|c|c}
% visual representation&vocab size & used words& sender & commun. success &purity & rand. purity & purity-rand. purity\\\hline
% probs & 100 & 58 & shared & 1.00 & 0.46        & 0.27 & 0.19\\
% fc & 100 & 38 & shared & 1.00 & 0.41           & 0.23 & 0.18\\
% probs & 10 & 10 & shared & 1.00 & 0.35         & 0.18 & 0.18\\
% fc & 10 & 10 & shared & 1.00 & 0.32            & 0.17 & 0.14\\
% probs & 100 & 2 & fullyconnected & 0.99 & 0.21 & 0.15 & 0.06\\
% fc & 10 & 2 & fullyconnected & 0.99 & 0.21     & 0.15 & 0.05\\
% probs & 10 & 2 & fullyconnected & 0.99 & 0.20  & 0.15 & 0.04\\
% fc & 100 & 2 & fullyconnected & 0.99 & 0.19    & 0.15 & 0.04\\
% \end{tabular}
% \label{tab:exp1_table}
% \caption{Table with results, no noise}
% \end{table}

\begin{table}
\centering
\begin{tabular}{c|c|c|c|c|c|c|c}
id & sender   &vis   &voc &used     &comm    &      purity ($\%$)   &obs-chance\\
 	&	& rep & size& symbols & success($\%$) &  & purity ($\%$) \\\hline
1&informed&probs     &100       &58          &100                &46           &0.27 \\
2&informed&fc        &100       &38          &100                &41           &0.23 \\
3&informed&probs     &10        &10          &100                &35           &0.18 \\
4&informed&fc        &10        &10          &100                &32           &0.17 \\
5&agnostic&probs     &100       &2           &99                 &21           &0.15 \\
6&agnostic&fc        &10        &2           &99                 &21           &0.15 \\
7&agnostic&probs     &10        &2           &99                 &20           &0.15 \\
8&agnostic&fc        &100       &2           &99                 &19           &0.15 \\
\end{tabular}
\label{tab:exp1_table}
\caption{Playing the referential game. \emph{Used symbols} column reports number of distinct vocabulary symbols that were produced at least once in the test phase. See text for explanation of \emph{comm success} and \emph{purity}. All purity values are highly significant ($p<0.001$) compared to simulated chance symbol assignment when matching observed symbol usage. %\textbf{Is this indeed the case? that is, is observed purity above the max chance value for all experiments reported in this table? if not, update accordingly. AL: YES, but I measured in your perl simulations how many times the chance purity was over the observed one.} 
The \emph{obs-chance purity} column reports the difference between observed purity and expected purity under chance.}
\end{table}

Table~\ref{tab:exp1_table} shows communication success for various configurations after 5k training rounds. Both sender architectures learn
to coordinate with the receiver. However, they have very different
qualitative behavior.  The informed sender, being encouraged to detect
pairwise relations between images, tends to make use of more symbols
from the available vocabulary, while the sender without this feature
coordinates using a very compact vocabulary. This might suggest that
the informed sender is using more varied and word-like symbols (recall
that the images depict about 463 objects, so we would expect a
natural-language-endowed sender to use a wider array of symbols to
discriminate among them). However, it could also be the case that the
informed sender vocabulary simply contains higher
redundancy/synonymy. Figure~\ref{fig:exp1_synonymy} plots the singular
values and spectral clustering of the informed sender symbol usage
(with fc input representations and 100 as  symbol vocabulary
size). We observe that, while there is some redundancy, the vocabulary
would not be able to get reduced to two symbols with the current
communication protocol.
\COMMENT{I did not follow the line of reasoning here: isn't the fact that the vocabulary could be reduced to two singular values a sign that it's indeed very redundant?} AL: Why do you  say that the vocabulary can be reduced to two symbols only? There is some information carried by the other dimensions as well.

\begin{figure}[tb]
\centering
\includegraphics[scale=0.35]{figures/singular}
\caption{Singular values and spectral clustering of symbols}
\label{fig:exp1_synonymy}
\end{figure}

\COMMENT{I am commenting out the
  former description and replacing it with one of what I did. Alex: if
  the description that follows is wrong, please reinstate yours.}

We now turn to investigating the semantic properties of the emergent
communication protocol. Recall that the vocabulary that agents use is
arbitrary and has no initial meaning. Thus, one way to look for the
emergence of high (vs.~low) level semantics is to look for the
relationship between symbols and the sets of images they refer to. To
look for these higher-level properties, we exploit the fact that the
objects in our images were categorized into \textbf{10} \textbf{AL: Why 10? We have 20...} broader
categories (such as \emph{weapon} and \emph{mammal}) by
\cite{McRae:etal:2005}. If the agents converged to intuitive meanings
for the symbols, we would expect that objects belonging to the same
category would activate the same symbols, e.g., that, say, when the
target images depict bayonets and guns, the sender would use the same
symbol to signal them. To quantify this, we associate each object to
the symbol that is most often activated when the target images contain
the object. We then assess the quality of the resulting symbol-based
clusters by measuring their \emph{purity} with respect to the McRae
categories. Purity \citep{Zhao:Karypis:2001} is a standard measure of
cluster quality, reaching 100\% for perfect clustering with respect to
the gold standard, and approaching 0 as cluster quality deteriorates.

Although purity is far from perfect, it is significantly above chance
in all cases, and we confirm that the informed-sender is producing
symbols that are more semantically natural than those of the agnostic
one. Perhaps surprisingly, purity is not at chance level even when
only two symbols are used. Qualitatively, in this case the agents seem
to converge to a (noisy) living-vs-non-living distinction, which,
intriguingly, has been recognized as the most basic one in the human
semantic system \citep{Caramazza:Shelton:1998}.

% We then compare this to the expected purity that we would get if class labels were randomly assigned to images. We see that the purity is higher than random, but that the clusters are not completely pure. 

% It is hard to interpret this measure as an absolute one, but we will show in our next experiment that interventions which we expect to raise the utilization of higher order features do, in fact, raise this measure as well.


% ALEX FROM HERE
% We now turn to investigating the natural language properties of the
% emergent communication protocol. Recall that the vocabulary that
% agents use is arbitrary and has no initial meaning. Thus, one way to
% look for the emergence of high (vs.~low) level semantics is to look
% for the relationship between symbols and the images they refer
% to.

% %[Discuss number of words used and whether that is necessarily high vs. low level]
% To look for these higher-level properties, we exploit the fact that
% each image that we work with already has an ImageNet class and there
% are many images in our set from each class. The basic idea is to ask
% whether we can use higher-level attributes of the image (e.g., whether
% the image is depicting a cat) to predict which vocabulary word the
% agents use to refer to it. If the agents are using low-level features
% (e.g., brightness in certain areas of the image), then we should be
% unable to do so.

% For every image, we look at the most commonly used word when that image is the target. We then treat the ImageNet class (eg. chair, fox, butterfly) as a clustering of images and compute the purity of the cluster by

% %[purity equation here]

% We then compare this to the expected purity that we would get if class labels were randomly assigned to images. We see that the purity is higher than random, but that the clusters are not completely pure. 

% It is hard to interpret this measure as an absolute one, but we will show in our next experiment that interventions which we expect to raise the utilization of higher order features do, in fact, raise this measure as well.
% ALEX TO HERE

\COMMENT{Assuming my description above is correct, I think the
  following is a different experiment, and this should be clarified}

We can visualize the clustering patterns as follows. For every
ImageNet class, we look at the symbol most commonly used by the sender
when an image of that class is the target. In addition, for each
class, we generate an embedding by averaging the embeddings of each
image in the class. We think this captures higher-level class
semantics for two reasons: first, the top layers of convolutional
neural networks are often thought to be expressing quite high-level
features of images \citep{Zeiler:Fergus:2014}. Second, if lower-level
features (e.g., brightness) are randomly assigned within class then
this averaging removes lower-level signals and leaves only higher
level ones.

\COMMENT{I don't understand the line of reasoning above. The aim of the current analysis is to show that the agents are converging to a meaningful code. In this perspective, what is the point of trying to use an external mechanism that is not part of agent's communication, namely averaging across images of objects? I think the latter should simply be justified as a way to improve the visualization, and not in virtue of any denoising function they might have. Perhaps, it would be even better to plot single images randomly selected?}

We then take these class embeddings and inspect if they form natural clusters and whether these clusters align with word usage. To see this, we perform a t-SNE mapping~\cite{Laurens:Hinton:2008} of the class embedding matrix, color-coded  by their majority symbol used. Figure \ref{fig:exp1_tsne} shows the result.

%\COMMENT{These plots should feature labels for a subset of the points, to let the reader understand what's going on.}

\begin{figure}[tb]
\centering
\includegraphics[scale=0.39]{figures/informed_fc_10_v1n0}
\includegraphics[scale=0.39]{figures/informed_fc_10_v1n1}
\caption{t-SNE plots of configurations without noise (\textbf{left}, 4th row of Table~\ref{tab:exp1_table}) and with noise (\textbf{right}, 2nd row of Table~\ref{tab:exp2_multiinstance}).}
\label{fig:exp1_tsne}
\end{figure}



==> framework_old.tex <==
\section{General Framework}
\label{sec:general-framework}

Our general framework includes: K players, each parametrized by their own $\theta_k$, a collection of tasks/games that the players have to perform, a communication protocol $V$ that enables the players to communicate with each other in order to solve the task and payoffs assigned to the players as a deterministic function of a well-defined goal. We focus for now on a specific problem: \textit{referential games} with the following structure:

\begin{enumerate}
\item There is a set of images represented by vectors $\lbrace i_1, \dots, i_N \rbrace$, two images are drawn at random from this set, call them $(i_L, i_R)$, one of them is chosen to be the ``target'' $t \in \lbrace L, R \rbrace$
\item There are two players, a sender and a receiver each seeing the images - the sender receives input $\theta_S (i_L, i_R, t)$
\item There is a \textit{vocabulary} $V$ of size $K$ and the sender chooses one symbol to send to the receiver, we call this the sender's policy $s(\theta_S (i_L, i_R, t))\in V$
\item The receiver does not know the target, but sees the sender's symbol and tries to guess the target image. We call this the receiver's policy $r(i_L, i_R, s(\theta_S (i_L, i_R, t))) \in \lbrace L, R \rbrace$ 
\item If $r(i_L, i_R, s(\theta_S (i_L, i_R, t)) = t$, that is, if the receiver gets the target correct, both players receive a payoff of 1 (win), otherwise they receive a payoff of 0 (lose).
\end{enumerate}

Many extensions to the basic referential game explored in this paper are possible. There can be more images, a more sophisticated communication protocol (e.g., communication of a sequence of symbols or multi-step ``20 questions''-style communication requiring back-and-forth interaction),  rotation of the sender and receiver roles, having a human occasionally playing one of the roles, etc. 

Our setup is an instance of the cheap talk games studied in game theory%~\citep{crawford1982strategic}
. These games have been used as models to study the evolution of language in simulations in the lab~\citep{crawford1998survey,blume:1998experimental} and theoretically~\cite{crawford1982strategic}. They are interesting because they strip away all structural properties of language and focus on  its functional properties only. In cheap talk games, communication is just one symbol and the symbols have no ex-ante semantics: meaning only emerges in the context of the game.

Game theory is traditionally concerned with the study of Nash equilibria: stable policy profiles that no agent can deviate from to increase their payoffs. Cheap talk games with sufficient expressiveness and common interest admit a Nash equilibrium where all private information that the sender knows is revealed to the receiver~\citep{crawford1982strategic}. Thus, the question for us is whether learning agents will converge to this equilibrium (as convergence in learning is not guaranteed: \citealt{fudenberg2014recency}).  In addition, there are many equilibria which have the same amount of information revelation. However, some of the languages that emerge from these equilibria may not be the ones we are looking for, ie. they may capture high level semantic properties of our images. We tackle this issue empirically below, by analyzing the ``meanings'' that our agents assign to the symbols they learn to use. 

\section{Experimental Setup}
\label{sec:experimental-setup}
%We instantiate our referential game as follows.

\paragraph{Images} We use the McRae et al.'s
(\citeyear{McRae:etal:2005}) set of 463 base-level concrete
concepts (e.g., \emph{cat, apple, car}\ldots) spanning across 20
general categories (e.g., \emph{animal}, \emph{fruit/vegetable},
\emph{vehicle}\ldots). We randomly sample 100 images of each concept
from ImageNet~\citep{Deng:etal:2009}. To create target/distractor
pairs, we randomly sample two concepts, one image for each concept and
whether the first or second image will serve as target. We apply to
each image a forward-pass through the pre-trained VGG ConvNet~\cite{Simonyan:Zisserman:2014}, and represent it with the activations from either
the last softmax layer (\emph{sm}) or the second-to-last fully
connected layer (\emph{fc}).
%
% We start with a set of concepts studied by ~\cite{McRae:etal:2005}, in the context of property norm generation. This set contains 541 base-level concrete concepts (e.g., cat, apple, car etc.) that span across 20 general and broad categories (e.g., animal, fruit/vegetable, vehicle etc). For the purposes of the current experiments, \textbf{X} McRae concepts were excluded (either because of high ambiguity or for technical reasons), resulting in \textbf{Y} concepts.
% For each concept, we randomly sample 100 images from its respective ImageNet~\cite{Deng:etal:2009}  entry.  
%\COMMENT{This would be a good place to describe how the images are
%  represented by passing them through pre-trained CNNs, using one of
%  two layers}

\paragraph{Agent Players} Both sender and receiver are simple
feed-forward networks.  For the sender, we experiment with the two
architectures depicted in Figure \ref{fig:players}. Both take as input
the target and distractor representations with a pointer to the
target. The \emph{agnostic} sender is a generic neural network that
maps the original image vectors onto a ``game-specific'' embedding
space followed by a sigmoid activation function, and then applies fully-connected weights to their concatenation
to produce scores over vocabulary symbols.\COMMENT{Comment for future work: have you tried adding one more
  hidden layer above the embedding concatenation?}  The
\emph{informed} sender, just like the agnostic one, first embeds the
images into a ``game-specific'' space. It then applies 1-D
convolutions (``filters'') on the image embeddings by treating them as
different channels (i.e., convolutions with kernel size 2x1), followed by a sigmoid activation function (in
Figure~\ref{fig:players}, there are 4 such filters). The resulting
feature maps are combined through another filter (kernel size fx1, where f is the number of bottom filters),  to produce scores for
the vocabulary symbols. 
Intuitively, the informed sender compares the two image embeddings
dimension-by-dimension. For both senders, motivated by the discrete
nature of language, we enforce a strong
communication bottleneck that discretizes the communication
protocol. Activations  on the top (vocabulary) layer 
%is normalized by
%the softmax transform
are converted to a Gibbs distribution 
(with temperature parameter $\tau$), and then a
single symbol $s$ is sampled from the resulting probability
distribution.

The receiver takes as input the target and distractor image vectors in
randomized order and the symbol produced by the sender (as a one-hot
vector over the vocabulary).  It also embeds the images, as well as
the symbol, onto its own ``game-specific'' space. It then computes dot
products between the symbol and image embeddings. Ideally, dot similarity should be higher for the image that is better denoted by the symbol. %
% Intuitively, the dot similarity will be higher for the image for which
% the symbol embedding is most active. 
The two dot products are %softmax-transformed
converted to a  Gibbs distribution 
 (again with temperature parameter $\tau$) and the
receiver ``points'' to an image by sampling from the resulting
probability distribution.%\COMMENT{I changed the descriptions of
 % sampling of both sender and receiver to avoid a notation that is
%  different from the one used in the General Framework. If you want to
 % re-instated the notation, please make it compatible with the
 % notation in that section (original chunks commented out but still in
 % the source).}
% Finally, the receiver performs the action of ``pointing'' to
% an image $i$ by sampling from a Gibbs distribution
% $p_{\theta_R}(o|i_L,i_R,s)$ (with temperature $\tau$) parametrized
% by the scores over the two images $o_1$ and $o_2$ produced by the
% receiver.
% from a Gibbs distribution $p_{\theta_S}
% (s|o_t,o_d)$ (with temperature $\tau$) parametrized by the symbol
% scores produced by the sender. This produced symbol is the message
% that the sender sends over to the receiver.


%\COMMENT{Have you tried different depths for FULLYCONNECTED?} AL: Probably??
% I see I repeat myself :)

%\COMMENT{A bit more details: how are the networks trained, and vocabulary size}

\begin{figure}
\includegraphics[scale=0.20]{figures/players}
\caption{Architectures of agent players.%\textbf{Any comments on there or they look ok? Put a frame around the target for the sender architectures. You can perhaps also grey out the 3d symbol of the senders, to clarify the link with the third input to the receiver.}
}
\label{fig:players}
\end{figure}

\paragraph{General Training Details} We set the following
hyperparameters without tuning: embedding dimensionality of all embedding matrices: 50, number of filters applied to embeddings by
  informed sender: 20, temperature of all Gibbs distributions: 10. We explore two vocabulary sizes: \emph{10} and
\emph{100} symbols. The sender and receiver parameters $\theta=\langle
\theta_{R}, \theta_{S}\rangle$ are learned jointly while playing the
game. The only supervision used is communication success, i.e.,
whether the agents agreed on the referent. This setup is naturally
modeled with Reinforcement Learning \citep{Sutton:Barto:1998}. As
outlined in Section \ref{sec:general-framework}, the sender follows policy $s(\theta_S (i_L, i_R, t))\in V$ and the receiver policy $r(i_L, i_R, s(\theta_S (i_L, i_R, t))) \in \lbrace L, R \rbrace$. The loss function that the two agents must minimize is  $-\Expect_{\tilde{r}} [R(\tilde{r})]$ where $R$ is the reward function returning 1 iff $r(i_L, i_R, s(\theta_S (i_L, i_R, t)) = t$. %
%  The agent parameters implement a
% \emph{policy}. By executing it, the agents perform
% \emph{actions}, i.e., the sender picks a symbol from the distribution
% $p_{\theta_S} (s|o_t,o_d)$ and the receiver points to an image by
% sampling from the distribution $p_{\theta_R} (o|o_1,o_2,s)$. The loss
% function that the two agents are minimizing is
% $-\Expect_{\tilde{o}\sim p(o|o_1,o_2,s)}[R(\tilde{o})]$, where $R$ is
% the reward function which returns 1 iff $\tilde{o} =$ target. 
Parameter are updated through the Reinforce rule~\cite{Williams:1992}.
We apply mini-batch updates, with a batch size of 32 and for a total of
50k iterations (games).  \textbf{At test time, we compile a set of 10k games  consisting of a target and a distractor by randomly sampling two objects and for each object an image.}

We now turn to our main questions. The first is whether the agents can
learn to successfully coordinate in a reasonable amount of time (as
there are plenty of examples where certain learning models are simply
unable to converge to Nash equilibria, given certain inputs
\textbf{(CITE)}). The second is whether the language that agents
converge to can be thought of as ``natural language'', in the sense
that symbols are assigned meanings that make intuitive sense in terms
of our conceptualization of the world.










==> introduction_old.tex <==
\section{Introduction}

%\COMMENT{I found the first paragraph somewhat out of place: in the
%  rest of the paper, we are focusing on communication and interaction,
%  whereas this paragraph is more about avoiding data labeling and
%  transfer learning. I have tentatively commented it out from here
%  (without editing it, and pasted an edited version at the end of the
%  introduction.}
% The dominant paradigm in AI is to train models on labeled examples. However, this paradigm is data intensive and agents trained in this way are hard to port to even slightly different tasks (cite something about Yann talking about how unsupervised learning will save all the things). Some modern research has adopted an evolutionary perspective to try to mitigate this hunger for data: learning can be bootstrapped from competition between agents. This has been shown to be successful in generative adversarial networks (GANs, \citealt{Goodfellow:etal:2014}) and in game playing (citealphago). In this paper, we argue that cooperation between multiple agents can also be used as a way to bootstrap learning and use this idea to propose a paradigm for natural language development.\footnote{Cooperation and coordination between multiple artificial agents is well studied, indeed the whole field of \textit{multiagent systems} (cite) is built on trying to induce it. However, we focus not on cooperation to achieve a task but cooperation \textit{as a learning tactic} to build agents with certain capabilities.}

One of the most ambitious goals in AI is to develop agents that can cooperate with others to achieve goals \citep{wooldridge2009introduction}. Such coordination is impossible without communication, and, if the coordination partners are to include humans, the most natural channel of communication is natural language. Thus, handling natural-language-based communication is a key step toward the development of AI that can thrive in a world populated by other agents.

Given the success of deep learning models directly trained on end-task
examples in related domains such as image captioning or machine
translation \citep[e.g.,][]{Sutskever:etal:2014,Xu:etal:2015}, it
would seem reasonable to cast the problem of training conversational
agents as an instance of supervised learning from large collections of
conversations. However, training on \emph{canned} conversations does
not allow learners to experience the interactive aspects of
communication \citep{Vinyals:Le:2015}. This paradigm is an excellent
way to learn general statistical associations between sequences of
symbols, but it focuses on the structure of language rather than on
its purpose, that is, the fact that we use words to make things happen
\citep{Austin:1962,clark1996using}.

The functional view of language was notably explored by Wittgenstein in his Philosophical Investigations \citep{Wittgenstein:1953}. In a key example, Wittgenstein argues that children do not learn language merely by observation and annotation. When a child looks at her mother and says ``bottle'', she is not only pointing out the bottle or repeating her mother’s utterance, she is asking for something to drink. Here, the child is learning language in order to coordinate her actions with her mother in order to get things done.

In this paper we propose a research program based on
\textit{multi-agent coordination communication games}. These games
place agents in simple environments where they need to coordinate
through communication to earn payoffs. Instead of learning to
reproduce existing patterns, the agents develop a shared language in
order to maintain coordination. Importantly, multiple agents start as
tabulae rasae but play the games together. In this way, they can
develop and bootstrap knowledge on top of each other. The central
problem of our program is the following: How do we design environments
fostering the development of a language that is portable to new
situations and communication partners (in particular
humans)? % The goal of this paper is to begin to understand the minimal
% features of learning environments that cause coordinating agents to
% develop languages with various properties.

Other researchers have proposed communication-based environments for
the development of AIs capable of coordination. We view our paradigm
as complementary to the existing
literature. %We try to borrow the good qualities from each approach while minimizing their downsides.
Work in multi-agent systems has focused on the design of
pre-programmed communication systems to solve specific tasks (e.g.,
robot soccer \citep{stone1998towards}). \cite{sukhbaatar2016learning}
show that neural networks are flexible enough that they do not require
pre-coded communication protocols, but they can evolve communication
in the context of the game.%\footnote{The literature on the emergence
  %of language in linguistics and cognitive science has also shown that
  %neural-network-based agents can evolve a language for coordination
  %(cite), though the environments considered in that tradition are
  %much simpler than those of \cite{sukhbaatar2016learning}.} 
  We also
exploit the flexibility of neural networks as building blocks for our
communicating agents. \cite{sukhbaatar2016learning} study whether the
language emerging in their games is interpretable with mixed
results. We pursue the same question, but pushing it one step further
by asking how we can change our game to make the emergent language
more interpretable.

The SHRLDU program of \citealt{Winograd:1971} was a prime example of
building an AI that can communicate with
humans.\footnote{\citealt{Wang:etal:2016}), who study coordination in
  simple ``task accomplishment'' games, are a more recent example of a
  similar approach.} To do this, it puts humans in the loop from the
very beginning. While attractive, this idea faces serious scalability
issues, as active human intervention is required at each step of
training. We would like to get the benefits of a human in the loop at
lower costs. Our general paradigm is however flexible enough that we
could also consider variants in which human agents participate in
referential games with machines from the very beginning.

A third branch of research focuses on ``Wizard-of-Oz'' environments,
where %artificial 
agents learn to play games by interacting with a
complex scripted environment~\citep{Mikolov:etal:2015a}. This approach
gives the designer tight control over the learning curriculum, but 
imposes a heavy engineering burden on the developers. We also stress
the importance of the learning environment, but we focus on simpler
setups and try to make our agents get smarter by bootstrapping on top
of each other.

Our approach also allows us to leverage ideas from work in
linguistics, cognitive science and game theory on the emergence of
language (see, e.g., \citealt{Wagner:etal:2003,Skyrms:2010,
  crawford1982strategic,crawford:1998survey}). We take inspiration from this work, but we also note that it mostly focuses on simple models to \textit{learn about} properties of existing language while we focus on more fleshed out input data and neural networks in order to \textit{engineer} communicating agents.

An evolutionary perspective has also recently been advocated as a way
to mitigate the data hunger of traditional supervised approaches:
Learning can be bootstrapped from \emph{competition} between
agents. This has been shown to be successful in generative adversarial
networks \citep{Goodfellow:etal:2014} and in game playing
\citep{Silver:etal:2016}. The \emph{cooperative} setup we propose can
also be seen as a way to foster learning while reducing the need for
annotated data.  

Cooperation and coordination between multiple artificial agents is well-studied in the field of \textit{multiagent systems}~\cite{Shoham:LeytonBrown:2009}. However, in this work, we focused on cooperation \textit{as a learning tactic}, rather as a means to achieve a task.  



==> related_work.tex <==
\section{Related Work}
One advantage of our framework is that it is highly related to existing work in the fields of linguistics and game theory. These fields are mostly concerned with asking how language develops rather than trying to engineer intelligent agents, however, it seems fruitful to leverage decades of work to inform our efforts. We give two notable examples next.

\paragraph{Game theory}
There is a large literature in game theory (\cite{farrell:1996}, \cite{blume:1998experimental}, \cite{crawford:1998survey}, \cite{Skyrms:2010}) and theoretical biology (\cite{nowak:2006evolutionary}) that focuses on signaling games. These are games of asymmetric information where one player ``knows'' something the other does not and has incentives to either reveal or not reveal it. One important strand of this literature concerns ``cheap talk'' games where agents must coordinate on some actions and have access to communication which initially has no meaning but gains meaning in the Nash equilibria of the game. Work in this literature focuses on understanding the theory of such games (\cite{farrell:1996}), whether learning or evolution can solve them (\cite{nowak:2006evolutionary}) and whether humans can learn to communicate and coordinate in laboratory settings (\cite{crawford:1998survey}, \cite{blume:1998experimental}).

\paragraph{Language evolution}
The field of language evolution is also closely related to the proposed framework. In the early and mid 1990's large groups of researchers were interested in multi-agent communication simulations using neural networks (\cite{Kirby:Hurford:2002},\cite{Steels:2015}) . While there is much there to be learned for our situation, given the focus of these works on studying the origins of language, the simulations from this period were rather restricted with respect to the nature and size of of input data, i.e, mostly artificial input and small networks (see ~\cite{Wagner:etal:2003} for a  comprehensive literature review on this field). In this position paper, we are arguing in favor of a multi-agent communication framework as the foundation of building machines that can communicate with us, thus focusing on more realistic data/input and less assumptions about their nature. 
